Empowering Interdisciplinary Insights with Dynamic Graph Embedding Trajectories

We developed DyGETViz, a novel framework for effectively visualizing dynamic graphs (DGs) that are ubiquitous across diverse real-world systems. This framework leverages recent advancements in discrete-time dynamic graph (DTDG) models to adeptly handle the temporal dynamics inherent in dynamic graphs. DyGETViz effectively captures both micro- and macro-level structural shifts within these graphs, offering a robust method for representing complex and massive dynamic graphs. The application of DyGETViz extends to a diverse array of domains, including ethology, epidemiology, finance, genetics, linguistics, communication studies, social studies, and international relations. Through its implementation, DyGETViz has revealed or confirmed various critical insights. These include the diversity of content sharing patterns and the degree of specialization within online communities, the chronological evolution of lexicons across decades, and the distinct trajectories exhibited by aging-related and non-related genes. Importantly, DyGETViz enhances the accessibility of scientific findings to non-domain experts by simplifying the complexities of dynamic graphs. Our framework is released as an open-source Python package for use across diverse disciplines. Our work not only addresses the ongoing challenges in visualizing and analyzing DTDG models but also establishes a foundational framework for future investigations into dynamic graph representation and analysis across various disciplines.

==> src/discussion.tex <==
\section{Discussion}
\label{sec:Discussion}
\yq{Should we include a section with this name? Or should we include this section into ``Conclusion'' or ``Experiments''?}

\subsection{Complexity Analysis}

The major additional cost in \model is the cosine similarity computation (Line~\ref{line:CosSim} in Alg.~\ref{alg:algorithm}), which has a time complexity of $O(N^2d)$. In practice, this can be performed using highly efficient tensor operations on GPU. 

Orthogonal Procrustes~\cite{hamilton2016diachronic} is an alternative measure. It consists of three parts. The cross-covariance matrix computation takes $O(ND^2)$. The singular value decomposition (SVD) takes $O(D^3)$. The rotation matrix is computed in $O(D^2)$. Therefore, the overall complexity is $O(ND^2 + D^3)$.





==> src/preliminary.tex <==
\section{Preliminary}
\label{sec:preliminary}

We present
% the problem of \problem\ as well as 
the necessary background and definitions. Notations in this paper are summarized in Supplementary Table~\ref{tab:notations}.
% \my{I think it would be better to switch the rows of $v_i$ and $\mathcal{N}(i, k, t)$ in Table~\ref{tab:notations} so that $v_i$ is defined before $\mathcal{N}(i, k, t)$}

\subsection{Graph}
% \yq{Expand on how DTDG works. Formulas}
A (static) graph, denoted as $G=(V, E)$, consists of a set of vertices (\aka, nodes) $V=\left\{v_1, v_2, \ldots, v_{|V|}\right\}$ and a set of edges (\aka, links) $E \subseteq V \times V$. To incorporate temporal information, dynamic graphs (DGs) are introduced, which can be classified as \emph{discrete-time dynamic graphs} (DTDGs) and \emph{continuous-time dynamic graphs} (CTDGs).
A DTDG~\cite{kazemi2020representation,seo2018structured,chen2022gc,TGC_ML} is a chronologically ordered sequence of graph snapshots, represented as $\left\{G^1, G^2, \ldots, G^T\right\}$. Each snapshot $G^t=\left\{V^t, E^t\right\}$ corresponds to the nodes $V^t \subseteq V$ and edges $E^t \subseteq E$ present at time $t$. 
On the other hand, a CTDG~\cite{wanginductive,rossi2020temporal,xu2020inductive,MNCI_ML_SIGIR} consists of a static graph $G$ representing the initial state of the dynamic graph at time $t=0$, and a set of graph events denoted as $O$. A graph event can involve the addition or deletion of nodes or edges, along with a timestamp. At each timestamp $t$, each node $v_i$ is associated with a node embedding $\textbf{v}_i^t$, representing its current state. A CTDG can be flexibly converted into a DTDG by partitioning the graph events into regular-spaced time intervals and combining the nodes and edges present in each interval into a graph snapshot. 
In the context of dynamic graphs, an embedding trajectory is defined as the sequence of node representations within the dynamic network model, which illustrates the evolution of a node over a specified time period. 
In this work, we focus on embedding trajectory visualization of DTDG due to their prevalence and generalization ability in modeling multiple real-world problems~\cite{sankar2020dysat,pareja2020evolvegcn,kazemi2020representation}. % A model developed for both CTDG and DTDG can be applied to the task of DTDG~\cite{kazemi2020representation}. 
% Our framework can be extended to CTDG by taking their node embeddings at regular time intervals. 
% \yc{need to describe why we focus on DTDG by taking hte  with some references.} 


\subsection{Projection Function for Visualization} 
% Such a projection is essential to create meaningful visualizations because human perception and cognition are limited when it comes to understanding information beyond three dimensions.
Given a set of high dimensional embeddings $\mathbf{X} = \{\mathbf{x}_i\}_{i=1}^N$, where $\mathbf{x}_i$ represents a node $v_i$'s $d$-dimensional vector, a projection function~\cite{cantareira2020generic,van2008visualizing} $f:\mathbb{R}^{N \times d} \rightarrow \mathbb{R}^{N \times p} (p << d)$ maps high dimensional data into lower-dimensional representations  and meanwhile, preserve the similarity relations between embeddings $\mathbf{X}$ in the projection $\mathbf{Z} = \{\mathbf{z}_1, \ldots, \mathbf{z}_{N}\}$. Example projection functions include Principal Component Analysis (PCA)~\cite{hotelling1933analysis}, t-Distributed Stochastic Neighbor Embedding (t-SNE)~\cite{van2008visualizing}, Multidimensional Scaling (MDS)~\cite{torgerson1952multidimensional}, and Uniform Manifold Approximation and Projection (UMAP)~\cite{mcinnes2018umap}. 
Typically, $p$ is set to $2$ or $3$ which can be perceived by humans. 
% One widely used technique is t-SNE~\cite{van2008visualizing}, which seeks to preserve the similarity between embeddings $\mathbf{X}$ in the projection $\mathbf{Z} = \{\mathbf{z}_1, \ldots, \mathbf{z}_{N}\}$. 

\subsection{Dynamic Graph Embedding Trajectories Visualization}

The problem of \problem takes a sequence of graph snapshots $\{G^t\}$ as inputs. The outputs are two folds, including (1) a collection of temporal node embeddings $\{\mathbf{V}^t\}_{t=1}^{T}$, where each embedding matrix $\mathbf{V}^t$ represents the state of all nodes at the given timestamp $t$; and (2) a visual representation $\mathcal{P}$ showing the embedding trajectories of nodes in $V$ over all timestamps $[1, T]$. 


% \yc{The problem definition is one of the important sections, and should be compiled and cleared. I still think the two outputs need to be explained in more detail. 
% For temporal node embeddings, it is easy to understand for those who know the DTDG models, but for those who don't, the current description falls short. 
% The definition of $\mathcal{P}$ is vague. For example, is it generated for each node, and if so, why do we only see embedding trajectories for a subset and not for all nodes? Is it an embedding vector that represents the change from one timestamp to another in a node?}
% \yc{Can we formally define $\mathcal{P}$?} 
% \model\ aims to effectively handle the challenges of the changing landscape of dynamic graphs. This includes the continuously changing node embeddings over time, the addition and deletion of nodes, and the evolving node-node proximity.
% where $\mathbf{V}^t=\{\mathbf{v}_{i}^t\}$ is the set of node embeddings for $V^t$ at time $t$, and $T$ is the total number of timestamps. 

==> src/tab-MacroLevelMeasure.tex <==
\begin{table}[!ht]
    \caption{Comparison of NARC and }
    \vspace{-0.2cm}
    \label{tab:MacroLevelMeasure}
    \centering
    \begin{tabular}{|l|l|l|l|l|l|l|l|}
    \hline
        ~ & Reddit & DGraphFin & HistWords-EN & HistWords-CN & Aging & Enron & Ant \\ \hline
        NARC & 0.174717 & 0.33229103 & 0.331606531 & 0.331512887 & 0.332101828 & 0.292288155 & 0.302969131 \\ \hline
        L1 & 39.42749198 & 5.149682879 & 17.24415287 & 18.66680861 & 2.436076317 & 11.25639903 & 2.172510541 \\ \hline
        L2 & 4.360034567 & 0.55138823 & 1.943986272 & 2.17042762 & 0.319406749 & 1.270918957 & 0.234486337 \\ \hline
    \end{tabular}
\end{table}
